Enhancing Physical Layer Communication Security through Generative AI with Mixture of Experts

AI technologies have become more widely adopted in wireless communications. As an emerging type of AI technologies, the generative artificial intelligence (GAI) gains lots of attention in communication security. Due to its powerful learning ability, GAI models have demonstrated superiority over conventional AI methods. However, GAI still has several limitations, including high computational complexity and limited adaptability. Mixture of Experts (MoE), which uses multiple expert models for prediction through a gate mechanism, proposes possible solutions. Firstly, we review GAI model's applications in physical layer communication security, discuss limitations, and explore how MoE can help GAI overcome these limitations. Furthermore, we propose an MoE-enabled GAI framework for network optimization problems for communication security. To demonstrate the framework's effectiveness, we provide a case study in a cooperative friendly jamming scenario. The experimental results show that the MoE-enabled framework effectively assists the GAI algorithm, solves its limitations, and enhances communication security.

==> review.tex <==
\section{Review}

\subsection{Anomaly detection}

\textbf{Admoe: Anomaly detection with mixture-of-experts from noisy label}s
\cite{zhao2023admoe} 2023

\textbf{Problem Statement / Research Question:} 
It is impossible to get a large number of clean labels due to the data sensitivity and the cost of annotation. Often there exists a large number of weak/noisy historical security rules designed for detecting malware from different perspectives. Though not as perfect as human annotations, they are valuable as they encode prior knowledge from past detection experiences. Also, although each noisy source may be insufficient for difficult AD tasks, learning them jointly may build competitive models as they tend to complement each other.

\textbf{Key ideas used / Gaps:}

In this work, they propose ADMoE a weakly-supervised approach for enabling anomaly detection algorithms to learn from\textbf{ multiple sets of noisy labels}. In a nutshell, ADMoE enhances existing neuralnetwork-based AD algorithms by Mixture-of-experts (MoE) network(s), which has a learnable gating function to activate different subnetworks (experts) based on the incoming samples and their noisy labels.

\textbf{Key Technique / Methodolgy:}

The proposed ADMoE can jointly learn from multiple sets of noisy labels with the majority of parameters shared, while providing specialization and scalability via experts. \textbf{Unlike existing noisy label learning approaches, ADMoE does not require explicit mapping from noisy labels to network parameters, providing better scalability and flexibility.} To encourage ADMoE to develop specialization based on the noisy sources, they use noisy labels as (part of the) input features with learnable embeddings to make the gating function aware of them.

\quad\\

\textbf{Mixture of experts with convolutional and variational autoencoders for anomaly detection} \cite{yu2021mixture}  2021

\textbf{Problem Statement / Research Question:} 

Most of the existing AD methods solely \textbf{based on the reconstruction errors or latent representation using a single low-dimensional manifold} are often not ideal for the image objects with complex background. However, modeling the data as a mixture of low-dimensional nonlinear manifolds is natural and promising for the classification of anomalies.

\textbf{Key ideas used / Gaps:}

In this study to realize the promise of \textbf{multi-manifold latent information} for AD, they propose a mixture of experts ensemble with two convolutional variational autoencoders (CVAEs) and convolution network (MEx-CVAEC) which explicitly learns manifold relationships of data that make use of multiple encoded detections.

\textbf{Key Technique / Methodolgy:}

The manifolds information are extracted using the CVAE which can be trained endto-end via back-propagation. Moreover, \textbf{to obtain more manifold information in the latent space, they map the reconstructions into the new low-dimensional latent space} in each CVAE using an encoder-decoder-encoder (EDE) pipeline . Furthermore, in order to obtain a quantitative index from the latent space which is used to measure whether the manifold of the latent space can represent the discriminative features of anomaly-free data, a tower structure is used in the mixture-of-expert model to assign a latent score to each latent representation.


\quad\\

\textbf{Deep autoencoding gaussian mixture model for unsupervised
anomaly detection}  \cite{zong2018deep}  2018

\textbf{Problem Statement / Research Question:} 

Unsupervised anomaly detection on multi- or high-dimensional data is of great importance in both fundamental machine learning research and industrial applications, for which \textbf{density estimation} lies at the core. Density estimation is that given a lot of input samples, anomalies are those ones residing in low probability density areas. Previous approaches mainly suffer from decoupled model learning with \textbf{inconsistent optimization goals} and \textbf{incapability of preserving essential information in the low-dimensional space}.

\textbf{Key ideas used / Gaps:}

In this paper, they propose Deep Autoencoding Gaussian Mixture Model (DAGMM). DAGMM preserves the key information of an input sample in a low-dimensional space that includes features from both the reduced dimensions discovered by dimensionality reduction and the induced reconstruction error.

\textbf{Key Technique / Methodolgy:}

Unlike the existing works, DAGMM extracts useful features for anomaly detection through non-linear dimensionality reduction realized by a deep autoencoder, and jointly learns their density under the GMM framework by \textbf{mixture membership estimation}, for which DAGMM can be viewed as a more powerful deep unsupervised version of adaptive mixture of experts in combination with a deep autoencoder. Moreover, DAGMM combines induced \textbf{reconstruction error and learned latent representation for unsupervised anomaly detection}.



\subsection{DoS attack}

\textbf{Real-time cbr-agent with a mixture of experts in the reuse stage to classify and detect dos attacks }\cite{pinzon2011real} 2011


\textbf{Problem Statement / Research Question:} 

Most proposed approaches focus only on ensuring confidentiality and integrity, without putting forward mechanisms that ensure the availability of services and resources offered like DoS attacks.


\textbf{Key ideas used / Gaps:}

This article presents a soft computing-based approach to cope with DoS attacks, but unlike existing solutions, the proposal \textbf{takes into account the different soft computing mechanisms} that can lead to a DoS attack.

\textbf{Key Technique / Methodolgy:}

The proposed approach is based on a \textbf{real time} classifier agent that incorporates a \textbf{mixture of experts} to choose a specific classification technique depending on the feature of the attack and the time available to solve the classification. With this scheme it is possible to divide the problem into subproblems, solving the classification of the web service requests in a more simple and effective way and always \textbf{within a time bound interval}.

\subsection{Spoofing}

\textbf{adaptive mixture of experts learning for generalizable face anti-spoofing} \cite{zhou2022adaptive} 2022

\textbf{Problem Statement / Research Question:} 

\textbf{Face anti-spoofing (FAS)} approaches based on \textbf{domain generalization (DG)} have drawn growing attention to improve the generalization. Existing DG-based FAS approaches always \textbf{capture the domain-invariant features for generalizing on the various unseen domains.} However, they \textbf{neglect individual source domains’ discriminative characteristics and diverse domain-specific information of the unseen domains}, and the trained model is not sufficient to be adapted to various unseen domains.

\textbf{Key ideas used / Gaps:}

They propose an \textbf{Adaptive Mixture of Experts Learning} (AMEL) framework, which exploits the domain-specific information to adaptively establish the link among the seen source domains and unseen target domains to further improve the generalization. 

\textbf{Key Technique / Methodolgy:}

\textbf{Domain-Specific Experts (DSE)} are designed to investigate discriminative and unique domain-specific features as a complement to common domain-invariant features. Moreover, \textbf{Dynamic Expert Aggregation (DEA)} is proposed to adaptively aggregate the complementary information of each source expert based on the domain relevance to the unseen target domain. And combined with meta-learning, these modules work collaboratively to adaptively aggregate meaningful domain-specific information for the various unseen target domains. 


\subsection{Phishing}

\textbf{A lightweight multi-view learning approach for phishing attack detection using transformer with mixture of experts }\cite{wang2023lightweight} 2023

\textbf{Problem Statement / Research Question:} 

Many machine learning-based methods for detecting phishing websites rely on URL analysis. However, these approaches are not always effective due to the following reasons: (1) highly concealed phishing websites may employ \textbf{tactics such as masquerading URL addresses} to deceive machine learning models, and (2) phishing attackers \textbf{frequently change} their phishing website URLs to evade detection.

\textbf{Key ideas used / Gaps:}

In this study, they proposed a robust, multi-view Transformer model with an \textbf{expert-mixture mechanism} for accurate phishing website detection utilizing website URLs, attributes, content, and behavioral information. 

\textbf{Key Technique / Methodolgy:}

They first adapted a pretrained language model for URL representation learning by applying adversarial post-training learning in order to \textbf{extract semantic information} from URLs. Next, they captured the attribute, content, and behavioral features of the websites and encoded them as vectors, which, alongside the URL embeddings, \textbf{constitute the website’s multi-view information}. Subsequently, they introduced \textbf{a mixture-of-experts mechanism into the Transformer network} to learn knowledge from different views and adaptively fuse information from various views. 


\subsection{High Rate Flooding Attacks}

\textbf{M2kmix: Identifying the type of high rate flooding attacks using a mixture of expert systems }\cite{arun2012m2kmix} 2012

\textbf{Problem Statement / Research Question:} 

These high rate flooding attacks deplete the \textbf{limited capacity of the server resources}. Existing detection techniques used in Firewalls, IPS, IDS, etc., \textbf{fail to identify the illegitimate traffic} due to its self-similarity nature of legitimate traffic and suffer from low detection accuracy and high false alarms. Also, very few in the literature have focused on \textbf{identifying the type of attac}k.

\textbf{Key ideas used / Gaps:}

This paper focuses on the \textbf{identification of type of high rate flooding attack} with High detection accuracy and fewer false alarms. The attack type identification is achieved by training the classifiers with different feature subsets. Therefore, \textbf{each trained classifier is an expert} in different feature space. High detection accuracy is achieved by creating a mixture of expert classifiers and the ensemble output decisions are identified by proposed Preferential Agreement (PA) rule. 

\textbf{Key Technique / Methodolgy:}

The proposed classification algorithm, M2KMix (mixture of two Multi Layer Perceptron and one K-Nearest Neighbor models) differs from the existing solutions in feature selection, error cost reduction, and attack type identification. 

\subsection{Federated learning}

\textbf{Federated learning using mixture of experts }\cite{zec2020federated} 2020

\textbf{Problem Statement / Research Question:} 

Current incarnations show limited privacy properties and have shortcomings when applied to common real-world scenarios. One such scenario is heterogeneous data among devices, \textbf{where data may come from different generating distributions}.

\textbf{Key ideas used / Gaps:}

They propose a federated learning framework using a \textbf{mixture of experts} to balance the specialist nature of a locally trained model with the generalist knowledge of a global model in a federated learning setting. 

\textbf{Key Technique / Methodolgy:}

Their framework includes a \textbf{personalized model for each client}, which is included in a mixture together with a globally trained model using federated learning. The local models never leave the clients, which gives strong privacy properties. Some clients can choose to opt-out from the federation, meaning that no information of their data is leaving the client, ensuring privacy of those clients.


\quad\\

\textbf{Pfl-moe: Personalized federated learning based on mixture of experts }\cite{guo2020pfl}

\textbf{Problem Statement / Research Question:} 

To cope with highly non-IID data distributions, personalized federated learning (PFL) has been proposed to improve overall performance by allowing each client to learn a personalized model. However, \textbf{one major drawback of a personalized model is the loss of generalization}. 

\textbf{Key ideas used / Gaps:}

To achieve model personalization while maintaining generalization, they propose PFL-MoE, which \textbf{mixes outputs of the personalized model and global model via the MoE architecture}. PFL-MoE is a generic approach and can be instantiated by integrating existing PFL algorithms. 

\textbf{Key Technique / Methodolgy:}

Particularly, they propose the PFL-MF algorithm which is an instance of PFL-MoE based on the \textbf{freeze-base PFL} algorithm. Then they further improve PFL-MF by enhancing the decision-making ability of MoE gating network and propose a variant algorithm PFL-MFE. The former is an instance of PFL-MoE and the later improves PFL-MF by modifying the MoE architecture so as to achieve better decision-making ability.

\quad\\

\textbf{Robust federated learning by mixture of experts }\cite{parsaeefard2021robust} 2021

\textbf{Problem Statement / Research Question:} 

FL is challenging due to the \textbf{non-IID nature of local data sets}.

\textbf{Key ideas used / Gaps:}

They present a novel \textbf{weighted average model based on the mixture of experts (MoE)} concept to provide robustness in FL against the poisoned/corrupted/outdated local models.

\textbf{Key Technique / Methodolgy:}

The server is equipped with public data set which can be applied to calculate the weighted average of models by optimization problems or predetermined roles such as softmax similar to MoE. 

\quad\\

\textbf{Byzantine-robust federated learning via server-side mixtue of experts }\cite{fan2023byzantine} 2023

\textbf{Problem Statement / Research Question:} 

Byzantine-robust Federated Learning focuses on mitigating the impact of malicious clients by developing robust algorithms that ensure reliable model updates while preserving privacy. However, these methods may not perform well and can even disrupt the normal process when \textbf{the amount of data on the server-side is limited or the structure of the model is complex}. 

\textbf{Key ideas used / Gaps:}

They address this challenge by introducing FLSMoE that utilizes a \textbf{Server-side Mixture of Experts}. The model parameters uploaded by individual clients are considered as expert models. 

\textbf{Key Technique / Methodolgy:}

Through the utilization of the gating unit within the MoE, even with low server-side data requirement, it is able to effectively identify and exclude malicious clients by \textbf{assigning appropriate weights to their contributions}. 

\subsection{ data integrity attacks (smart grid) }

\textbf{Locational detection of data integrity attacks with multi-gate mixture-of-experts in smart grid }\cite{fan16locational} 2016

\textbf{Problem Statement / Research Question:} 

Recent research has shown that a type of data \textbf{integrity attacks} named false data injection (FDI) attack can be launched against the state estimation while keeping stealthy to traditional mechanism. Attackers can modify estimated states by compromising measurements in system, causing severe consequences such as key lines overloading or load shedding. The presence detection or the detection of FDI attacks for whole system is\textbf{ a single-task classification problem}.

\textbf{Key ideas used / Gaps:}

The \textbf{multi-task classification problem} for locational detection of data integrity attacks is formulated in this paper. Based on the formulation, the locational detection with multi-gate mixture-of-experts (LD-MMoE) scheme is proposed.

\textbf{Key Technique / Methodolgy:}

Based on the formulation, a locational detection with \textbf{multi-gate mixture-of-experts (LD-MMoE) scheme} is proposed, which does not rely on additional conditions, e.g., the numbering sequence of measurements. LD-MMoE can greatly reduce the number of trainable parameters while keeping sufficient effectiveness.

\subsection{Bot detection}

\textbf{Botbuster: Multi-platform bot detection using a mixture of experts} \cite{ng2023botbuster} 2023

\textbf{Problem Statement / Research Question:} 

current bot detection models still face challenges in \textbf{dealing with incomplete data and a multi-platform bot detector}. It is near impossible to perform an extensive collection of all fields required by most bot detection algorithm, especially when there are at least a million accounts. Other times, it is simply impossible to collect all required data: the account may have been suspended or turned protected, forcing analysts to rely on available data or previously collected historical data.

\textbf{Key ideas used / Gaps:}

They advance the problem of bot detection modules through a mixture of experts architecture that can handle incomplete account information. Given an account’s information of username, screenname, description, user metadata, posts, where some information in this set may be missing, the goal is to classify the account into one of two classes: bot, human. 

\textbf{Key Technique / Methodolgy:}

Each expert is trained to analyze one pillar of data and are combined to estimate the probability that the account is a bot. The proposed solution, BotBuster, aims to overcome the limitations of requiring the entire set of account information for effective bot prediction and expand bot prediction to multi-platforms.

\subsection{Fake news detection}

\textbf{Collaborative mixture-of-experts model for multi-domain fake news detection }\cite{zhao2023collaborative} 2023

\textbf{Problem Statement / Research Question:} 

The growing spread of fake news on the Internet has become a serious threat to cyberspace and society at large. Most of existing methods focus on \textbf{single-domain fake-news detection}. Furthermore, any news content may belong to \textbf{multiple domains}.

\textbf{Key ideas used / Gaps:}

They propose a multi-domain fake-news detection framework based on \textbf{a mixture-of-experts model}.

\textbf{Key Technique / Methodolgy:}

 The input text is fed to BertTokenizer and embeddings are obtained by CLIP to obtain the fusion features. A sentiment module is used to analyze the inherent sentimental information of the text, and sentence-level and domain embeddings are used to form the collaboration module. Finally, the mixture-of-experts model, composed of TextCNN, is used to le\textbf{arn the features and construct a high-performance fake-news detection model}.

% \subsection{white-box adversarial attacks (image)}

% Self-routing capsule networks \cite{hahn2019self} 2019

% \textbf{Problem Statement / Research Question:} 



% \textbf{Key ideas used / Gaps:}



% \textbf{Key Technique / Methodolgy:}


\begin{table*}[htp]
    \caption{Summary of MoE methods for security }
    \centering
    \begin{tabular}{c|c|c|c|c}
        \hline
        Application & citations\\\hline
         Anomaly detection & \cite{zhao2023admoe} \cite{yu2021mixture} \cite{zong2018deep} \\\hline
         DoS attack & \cite{pinzon2011real} \\\hline
         Spoofing & \cite{zhou2022adaptive}  \\\hline
         Phishing & \cite{wang2023lightweight} \\\hline
         % Malware Detection & \cite{anantharamaiah2020malware}  \\\hline
          % vehicle prediction & \cite{mirus2019mixture} \\\hline
          High Rate Flooding Attacks  & \cite{arun2012m2kmix} \\\hline
          Federated learning & \cite{zec2020federated} \cite{parsaeefard2021robust} \cite{fan2023byzantine} \cite{zec2020specialized} \cite{guo2020pfl}\\\hline
          data integrity attacks (smart grid) & \cite{fan16locational} 
          \\\hline
          bot detection & \cite{ng2023botbuster} \\\hline
          % white-box adversarial attacks (image) & \cite{hahn2019self} \\\hline
          Fake news detection & \cite{zhao2023collaborative} \\\hline
          % Dataset & \cite{jain2024damex} \\\hline
          
        %\multicolumn{2}{c}{name}\\
    \end{tabular}
\end{table*}
